Reducing Minor Page Fault Overheads through Enhanced Page Walker

Application virtual memory footprints are growing rapidly in all systems from servers down to smartphones. To address this growing demand, system integrators are incorporating ever larger amounts of main memory, warranting rethinking of memory management. In current systems, applications produce page fault exceptions whenever they access virtual memory regions which are not backed by a physical page. As application memory footprints grow, they induce more and more minor faults. Handling of each minor fault can take few 1000's of CPU-cycles and blocks the application till OS finds a free physical frame. These page faults can be detrimental to the performance, when their frequency of occurrence is high and spread across application run-time. Specifically, lazy allocation induced minor page faults are increasingly impacting application performance. Our evaluation of several workloads indicates an overhead due to minor faults as high as 29% of execution time. In this paper, we propose to mitigate this problem through a hardware, software co-design approach. Specifically we first propose to parallelize portions of the kernel page allocation to run ahead of fault time in a separate thread. Then we propose the Minor Fault Offload Engine(MFOE), a per-core HW accelerator for minor fault handling. MFOE is equipped with pre-allocated page frame table that it uses to service a page fault. On a page fault, MFOE picks a pre-allocated page frame from this table, makes an entry for it in the TLB, and updates the page table entry to satisfy the page fault. The pre-allocation frame tables are periodically refreshed by a background kernel thread, which also updates the kernel memory management data-structures. We evaluate this system in the gem5 architectural simulator with a modified Linux kernel. Our results show that MFOE improves the average critical-path fault handling latency by 33x.

==> related-work.tex <==
\section{Related Work}
\label{sec:related}

%IT LOOKS LIKE THIS SECTION REPEATS MUCH OF WHAT IS ALREADY IN THE BACKGROUND SECTION --COMBINE THIS INTO THAT SECTION.

\subsection{Hardware Paging}
Recent work \cite{sigarch20} advocated hardware based demand paging for major page faults. This work has similar motivation as our work, in reducing the cost of page faults, but focuses on major page faults. Our work here showed the importance of handling minor page faults even when the data sets can be entirely memory resident. Nevertheless, our approach could be extended to support major faults. In contrast to single pre-allocation queue proposed in that work, we have proposed a  per-core pre-allocation tables, this would be flexible to implement NUMA policy on pre-allocated pages.

\cite{pemberton2018enabling} observed major page-fault handling latency becoming an overhead, when it is used as a mechanism to fetch pages from disaggregated memory node. Their approach is similar to ours i.e. they have offloaded fault handling to HW accompanied by kernel changes. But their system is designed to accelerate disaggregate memory faults, but not minor page-faults. 

\cite{10.1145/3037697.3037710} proposes adding  page-fault support to network controllers to avoid page pinning for DMA requests. Our page-fault handling mechanism is orthogonal to this proposal and can be integrated with this work, to enhance the fault handling latency.
\cite{guo2021clio} proposes hardware based page-fault handler for its virtual memory implementation at disaggregated memory node. This proposal focuses on implementing light weight virtual memory for remote memory accesses with offloading of fast path to ASIC \& FPGA, and slow path to ARM processor, in co-designed memory node. Albeit the design similarities, this proposal is unrelated to our approach in this paper. Our approach focuses on offloading generic anonymous fault handling to enhanced page table walker.

\subsection{Paging Optimization}
Large pages have been proposed to reduce the costs of number of page faults to be handled \cite{LargePage1,LargePage2,range-translations,LargePage-Ingens} and sometimes to increase the reach of the TLBs \cite{TLB-extend1}. Large pages are beneficial when addresses are allocated over contiguous ranges, but many new applications allocate small objects \cite{FB-workload}, and have required additional support for efficiencies \cite{perforated-pages}. Our approach here works across different workloads and moves much of the memory management overhead away from inline processes. 
Mitosis\cite{10.1145/3373376.3378468} replicates page table entries in multi-node systems, to avoid costly remote accesses during page table walks by HW page table walker. Our approach makes uses of hardware page table walker, but doesn't put any restriction on page table entry placement. Hence, MFOE can be made to work with Mitosis. 
\subsection{Miscellaneous}
\cite{203151} proposes tracking PTE access bits to avoid unnecessary TLB shoot-downs.  Our enhanced hardware page table walker, sets the PTE access bit during both  page walk, and page fault handling in hardware. Hence no disruption to the page access tracking mechanism is caused by our enhanced page table walker.
Prefetching has also been proposed to reduce the cost of misses on page accesses \cite{SPAN, Translation-prefetching}. Prefetching is complementary and can work with our approach. 
